Matrix factorization ranks via polynomial optimization

In light of recent data science trends, new interest has fallen in alternative matrix factorizations. By this, we mean various ways of factorizing particular data matrices so that the factors have special properties and reveal insights into the original data. We are interested in the specialized ranks associated with these factorizations, but they are usually difficult to compute. In particular, we consider the nonnegative-, completely positive-, and separable ranks. We focus on a general tool for approximating factorization ranks, the moment hierarchy, a classical technique from polynomial optimization, further augmented by exploiting ideal-sparsity. Contrary to other examples of sparsity, the resulting sparse hierarchy yields equally strong, if not superior, bounds while potentially delivering a speed-up in computation.

==> references.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%
%\biblstarthook{References may be \textit{cited} in the text either by number (preferred) or by author/year.\footnote{Make sure that all references from the list are cited in the text. Those not cited should be moved to a separate \textit{Further Reading} section or chapter.} If the citatiion in the text is numbered, the reference list should be arranged in ascending order. If the citation in the text is author/year, the reference list should be \textit{sorted} alphabetically and if there are several works by the same author, the following order should be used:
%\begin{enumerate}
%\item all works by the author alone, ordered chronologically by year of publication
%\item all works by the author with a coauthor, ordered alphabetically by coauthor
%\item all works by the author with several coauthors, ordered chronologically by year of publication.
%\end{enumerate}
%The \textit{styling} of references\footnote{Always use the standard abbreviation of a journal's name according to the ISSN \textit{List of Title Word Abbreviations}, see \url{http://www.issn.org/en/node/344}} depends on the subject of your book:
%\begin{itemize}
%\item The \textit{two} recommended styles for references in books on \textit{mathematical, physical, statistical and computer sciences} are depicted in ~\cite{science-contrib, science-online, science-mono, science-journal, science-DOI} and ~\cite{phys-online, phys-mono, phys-journal, phys-DOI, phys-contrib}.
%\item Examples of the most commonly used reference style in books on \textit{Psychology, Social Sciences} are~\cite{psysoc-mono, psysoc-online,psysoc-journal, psysoc-contrib, psysoc-DOI}.
%\item Examples for references in books on \textit{Humanities, Linguistics, Philosophy} are~\cite{humlinphil-journal, humlinphil-contrib, humlinphil-mono, humlinphil-online, humlinphil-DOI}.
%\item Examples of the basic Springer Nature style used in publications on a wide range of subjects such as \textit{Computer Science, Economics, Engineering, Geosciences, Life Sciences, Medicine, Biomedicine} are ~\cite{basic-contrib, basic-online, basic-journal, basic-DOI, basic-mono}. 
%\end{itemize}
%}

\begin{thebibliography}{99.}%

%\begin{thebibliography}{10}

\bibitem{Andersen2000}
E.~D. Andersen and K.~D. Andersen.
\newblock The {{MOSEK}} interior point optimizer for linear programming: {{An}}
  implementation of the homogeneous algorithm.
\newblock In H.~Frenk, K.~Roos, T.~Terlaky, and S.~Zhang, editors, {\em High
  Performance Optimization}, pages 197--232. {Springer US}, {Boston, MA}, 2000.

\bibitem{doi:10.1142/5273}
A.~Berman and N.~{Shaked-Monderer}.
\newblock {\em Completely Positive Matrices}.
\newblock {WORLD SCIENTIFIC}, 2003.

\bibitem{doi:10.1137/141000671}
J.~Bezanson, A.~Edelman, S.~Karpinski, and V.~B. Shah.
\newblock Julia: {{A}} fresh approach to numerical computing.
\newblock {\em SIAM Review}, 59(1):65--98, 2017.

\bibitem{BOMZE2014208}
I.~M. Bomze, W.~Schachinger, and R.~Ullrich.
\newblock From seven to eleven: {{Completely}} positive matrices with high
  cp-rank.
\newblock {\em Linear Algebra and its Applications}, 459:208--221, 2014.

\bibitem{doi:10.1137/140973207}
I.~M. Bomze, W.~Schachinger, and R.~Ullrich.
\newblock New lower bounds and asymptotics for the cp-rank.
\newblock {\em SIAM Journal on Matrix Analysis and Applications}, 36(1):20--37,
  2015.

\bibitem{10.1145/362342.362367}
C.~Bron and J.~Kerbosch.
\newblock Algorithm 457: {{Finding}} all cliques of an undirected graph.
\newblock {\em Communications of The Acm}, 16(9):575--577, Sept. 1973.

\bibitem{burerCopositiveRepresentationBinary2009}
S.~Burer.
\newblock On the copositive representation of binary and continuous nonconvex
  quadratic programs.
\newblock {\em Mathematical Programming}, 120(2):479--495, Sept. 2009.

\bibitem{Curto1996SolutionOT}
R.~E. Curto and L.~A. Fialkow.
\newblock Solution of the truncated complex moment problem for flat data.
\newblock 1996.

\bibitem{Curto2000TheTC}
R.~E. Curto and L.~A. Fialkow.
\newblock The truncated complex -moment problem.
\newblock {\em Transactions of the American Mathematical Society},
  352:2825--2855, 2000.

\bibitem{Klerk2019ASO}
E.~{de Klerk} and M.~Laurent.
\newblock A survey of semidefinite programming approaches to the generalized
  problem of moments and their error analysis.
\newblock {\em Association for Women in Mathematics Series}, 2019.

\bibitem{DelasCuevas2019separabilitymixed}
G.~{De las Cuevas}, T.~Drescher, and T.~Netzer.
\newblock Separability for mixed states with operator {{Schmidt}} rank two.
\newblock {\em Quantum}, 3:203, Dec. 2019.

\bibitem{delasCuevas2020MixedSI}
G.~{de las Cuevas} and T.~Netzer.
\newblock Mixed states in one spatial dimension: {{Decompositions}} and
  correspondence with nonnegative matrices.
\newblock {\em Journal of Mathematical Physics}, 2020.

\bibitem{Dickinson2014OnTC}
P.~J.~C. Dickinson and L.~Gijben.
\newblock On the computational complexity of membership problems for the
  completely positive cone and its dual.
\newblock {\em Computational Optimization and Applications}, 57:403--415, 2014.

\bibitem{doi:10.1080/09500340008244049}
D.~P. Divincenzo, B.~M. Terhal, and {Ashish V. Thapliyal}.
\newblock Optimal decompositions of barely separable states.
\newblock {\em Journal of Modern Optics}, 47(2-3):377--385, 2000.

\bibitem{Drew1994CompletelyPM}
J.~H. Drew, C.~R. Johnson, and R.~Loewy.
\newblock Completely positive matrices associated with {{M-matrices}}.
\newblock {\em Linear \& Multilinear Algebra}, 37:303--310, 1994.

\bibitem{Dunning2017JuMPAM}
I.~Dunning, J.~Huchette, and M.~Lubin.
\newblock {{JuMP}}: {{A}} modeling language for mathematical optimization.
\newblock {\em Siam Review}, 59:295--320, 2017.

\bibitem{fawziPositiveSemidefiniteRank2015}
H.~Fawzi, J.~Gouveia, P.~A. Parrilo, R.~Z. Robinson, and R.~R. Thomas.
\newblock Positive semidefinite rank.
\newblock {\em Mathematical Programming}, 153(1):133--177, Oct. 2015.

\bibitem{fawziSelfscaledBoundsAtomic2016a}
H.~Fawzi and P.~A. Parrilo.
\newblock Self-scaled bounds for atomic cone ranks: Applications to nonnegative
  rank and cp-rank.
\newblock {\em Mathematical Programming}, 158(1):417--465, July 2016.

\bibitem{Gharibian2010StrongNO}
S.~Gharibian.
\newblock Strong {{NP-hardness}} of the quantum separability problem.
\newblock {\em Quantum Information \& Computation}, 10:343--360, 2010.

\bibitem{doi:10.1137/1.9781611976410}
N.~Gillis.
\newblock {\em Nonnegative Matrix Factorization}.
\newblock {Society for Industrial and Applied Mathematics}, {Philadelphia, PA},
  2020.

\bibitem{Gribling2019LowerBO}
S.~Gribling, D.~{de Laat}, and M.~Laurent.
\newblock Lower bounds on matrix factorization ranks via noncommutative
  polynomial optimization.
\newblock {\em Foundations of Computational Mathematics}, pages 1--58, 2019.

\bibitem{Gribling2022BoundingTS}
S.~Gribling, M.~Laurent, and A.~Steenkamp.
\newblock Bounding the separable rank via polynomial optimization.
\newblock {\em Linear Algebra and its Applications}, 2022.

\bibitem{10.1145/780542.780545}
L.~Gurvits.
\newblock Classical deterministic complexity of {{Edmonds}}' problem and
  quantum entanglement.
\newblock In {\em Proceedings of the Thirty-Fifth Annual {{ACM}} Symposium on
  Theory of Computing}, {{STOC}} '03, pages 10--19, {New York, NY, USA}, 2003.
  {Association for Computing Machinery}.

\bibitem{Henrion2005}
D.~Henrion and J.-B. Lasserre.
\newblock Detecting global optimality and extracting solutions in
  {{GloptiPoly}}.
\newblock In D.~Henrion and A.~Garulli, editors, {\em Positive Polynomials in
  Control}, pages 293--310. {Springer Berlin Heidelberg}, {Berlin, Heidelberg},
  2005.

\bibitem{Korda2022ExploitingII}
M.~Korda, M.~Laurent, V.~Magron, and A.~Steenkamp.
\newblock Exploiting ideal-sparsity in the generalized moment problem with
  application to matrix factorization ranks.
\newblock 2022.

\bibitem{doi:10.1142/p665}
J.~B. Lasserre.
\newblock {\em Moments, Positive Polynomials and Their Applications}.
\newblock {IMPERIAL COLLEGE PRESS}, 2009.

\bibitem{Laurent2009}
M.~Laurent.
\newblock Sums of squares, moment matrices and optimization over polynomials.
\newblock In M.~Putinar and S.~Sullivant, editors, {\em Emerging Applications
  of Algebraic Geometry}, pages 157--270. {Springer New York}, {New York, NY},
  2009.

\bibitem{Lee1999LearningTP}
D.~D. Lee and H.~S. Seung.
\newblock Learning the parts of objects by non-negative matrix factorization.
\newblock {\em Nature}, 401:788--791, 1999.

\bibitem{doi:10.1137/1.9781611970791}
Y.~Nesterov and A.~Nemirovskii.
\newblock {\em Interior-Point Polynomial Algorithms in Convex Programming}.
\newblock {Society for Industrial and Applied Mathematics}, 1994.

\bibitem{10.1007/s10208-014-9225-9}
J.~Nie.
\newblock The {{A-truncated K-moment}} problem.
\newblock {\em Foundations of Computational Mathematics}, 14(6):1243--1276,
  Dec. 2014.

\bibitem{ShakedMondererCopositiveAC}
N.~{Shaked-Monderer} and A.~Berman.
\newblock {\em Copositive and Completely Positive Matrices}.
\newblock {World Scientific Publishing}.

\bibitem{ShakedMonderer2013OnTC}
N.~{Shaked-Monderer}, I.~M. Bomze, F.~Jarre, and W.~Schachinger.
\newblock On the cp-rank and minimal cp factorizations of a completely positive
  matrix.
\newblock {\em SIAM Journal on Matrix Analysis and Applications}, 34:355--368,
  2013.

\bibitem{Vavasis2009OnTC}
S.~A. Vavasis.
\newblock On the complexity of nonnegative matrix factorization.
\newblock {\em SIAM Journal on Optimization}, 20:1364--1377, 2009.

\bibitem{Yannakakis1988ExpressingCO}
M.~Yannakakis.
\newblock Expressing combinatorial optimization problems by linear programs.
\newblock In {\em {{STOC}} '88}, 1988.

\end{thebibliography}


